Off-shell vertices in heavy particle effective theories and $B\rightarrow D\pi \ell \nu$

We study the modifications to decay amplitudes in heavy to heavy semileptonic decays with multiple hadrons in the final state due to intermediate heavy hadrons being off-shell or having a finite width. Combining Heavy Hadron Chiral Perturbation Theory (HH$\chi$PT) with a BCFW on-shell factorization formula, we show that these effects induce $O(1/M)$ corrections to the standard results computed in the narrow-width approximation and therefore are important in extracting form factors from data. A combination of perturbative unitarity, analyticity, and reparameterization invariance fully determine these corrections in terms of known Isgur-Wise functions without the need to introduce new form factors. In doing so, we develop a novel technique to compute the boundary term at complex infinity in the BCFW formula for theories with derivatively coupled scalars. While we have used the $\bar B\rightarrow D\pi \ell\nu$ decay as an example, these techniques can generally be applied to effective field theories with (multiple) distinct reference vectors.

==> temp.tex <==
%
\section{Explicit solution for off-shell residual momentum \label{explicit-soln}} 
%
To find a solution for $q_\mu$ which satisfies $q\cdot p_{\ell \nu}=0$, $q\cdot p_\pi=0$, and $q^2=0$ it is convenient to choose a simple reference frame. A natural choice is the rest-frame of the meson which is pushed off-shell by the pion emission. We therefore take, without loss of generality, 
%
\begin{align}
    p_{\ell\nu} &= (E_{\ell\nu},0,0,P_{\ell\nu} )\\
    p_\pi       &= (E_\pi, P_\pi s_\theta ,0, P_\pi c_\theta) 
\end{align}
%
This then gives two solutions up to a re-scaling by some complex number $\mathfrak{z}$~,
%
\begin{equation}
    q=\mathfrak{z}\bigg(1,~~
    \frac{E_\pi}{P_{\pi }s_{\theta }}-\frac{ E_{\ell\nu}c_{\theta }}{P_{\ell\nu}s_{\theta }},~~
    \pm \iu \frac{\left(E_\pi P_{\ell\nu}-P_{\pi }  E_{\ell\nu}c_{\theta }\right) \sqrt{\frac{P_{\pi }^2 s_{\theta }^2 m_{\ell\nu}^2}{\left(P_{\pi } E_{\ell\nu}c_{\theta } -E_\pi P_{\ell\nu}\right){}^2}+1}}{P_{\pi } P_{\ell\nu} s_{\theta }},~~
    \frac{E_{\ell\nu}}{P_{\ell\nu}}\bigg)~,
\end{equation}
%
